Density dependence of the quark condensate in isospin-asymmetric nuclear matter

We compute the density dependence of the quark condensate and how it changes under the influence of isospin-asymmetric nuclear matter. This is achieved by the calculation of the relevant Feynman diagrams using in-medium chiral perturbation theory. We find that the absolute value of the quark condensate decreases in nuclear matter by around 35% at normal nuclear density, in agreement with previous model-independent calculations. We also present an quantitative estimation of the difference of up- and down quark in-medium condensates.

==> Condensate v3/feynman.tex <==
\newcommand{\len}[0]{1.0}


\tikzset{
  gluon/.style={thick, decorate, decoration={coil, amplitude=.08cm, segment length=.15cm, aspect=.75}}}
\tikzset{pion/.style={
	dashed,
	postaction={decorate},
	decoration={markings,mark=at position .6 with {\arrow{>}}}
	}}
\tikzset{nucleon/.style={
	postaction={decorate},
	decoration={markings,mark=at position .6 with {\arrow{>}}}
	}}
\tikzset{inmedium/.style={
	very thick,
	% postaction={decorate},
	% decoration={markings,mark=at position .55 with {\arrow{>}}}
	}}
\tikzset{source/.style={
	decorate,
	decoration={snake,amplitude=0.8mm}
	}}
\newcommand{\vertex}[2]{
	\fill[black!5] (#1) circle (.2);
	\draw (#1) circle (.2);
	\node at (#1) {\scalebox{0.8}{$#2$}};
}
\newcommand{\vertexVac}[1]{
	\fill[black] (#1) circle (.05);
	\draw (#1) circle (.05);
}
\tikzset{>=latex}
\usetikzlibrary{datavisualization}
\usetikzlibrary{datavisualization.formats.functions}
\usetikzlibrary{patterns}    	             % Schattierung in tikz
\usetikzlibrary{decorations.markings}        % for Feynman diagrams with tikz
\usetikzlibrary{shapes.geometric}            % for Feynman diagrams with tikz
\usetikzlibrary{decorations.pathmorphing}    % for decoration "snake"
\usetikzlibrary{decorations}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CONDENSATE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\CondensateSigma}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (C2) at ($(C)+(\len,0)$);
  \coordinate (C3) at ($(C2)+(\len,0)$);
  \draw[source] (A) -- (B);
  \draw[pion] (B) -- (C); 
  \draw[pion] (C) -- (C2);
  \draw[source] (C2) -- (C3);
  \vertex{B}{2};
  \vertex{C2}{2};
  \fill[black!5] (C) circle (.3);
  \draw (C) circle (.3);
}

\newcommand{\CondensateTypeOne}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (D) at ($(C)+(\len,0)$);
  \draw[source] (A) -- (B);
  \draw[source] (C) -- (D);
  \draw[double] ($(B)!0.5!(C)$) circle (.5cm);
  \node at ($(B)!0.5!(C)+(0,.5)$) {\scalebox{0.7}{$\blacktriangleright$}};
  \node at ($(B)!0.5!(C)-(0,.5)$) {\scalebox{0.7}{$\blacktriangleleft$}};
}

\newcommand{\CondensateTypeOnePi}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (D) at ($(C)+(\len,0)$);
  \coordinate (E) at ($(D)+(\len,0)$);
  \draw[source] (A) -- (B);
  \draw[pion] (C) -- (D);
  \draw[source] (D) -- (E);
  \draw[double] ($(B)!0.5!(C)$) circle (.5cm);
  \node at ($(B)!0.5!(C)+(0,.5)$) {\scalebox{0.7}{$\blacktriangleright$}};
  \node at ($(B)!0.5!(C)-(0,.5)$) {\scalebox{0.7}{$\blacktriangleleft$}};
  \vertex{D}{2};
}

\newcommand{\CondensateTypeTwo}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (D) at ($(B)+(0,-0.6)$);
  \draw[source] (A) -- (B);
  \draw[source] (B) -- (C);
  \draw[inmedium] ($(B)!0.5!(D)$) circle (.3cm);
  \node at (D) {\scalebox{0.7}{$\blacktriangleright$}};
}

\newcommand{\CondensateTypeTwoPi}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (C2) at ($(C)+(\len,0)$);
  \coordinate (D) at ($(B)+(0,-0.6)$);
  \draw[source] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[source] (C) -- (C2);
  \draw[inmedium] ($(B)!0.5!(D)$) circle (.3cm);
  \node at (D) {\scalebox{0.7}{$\blacktriangleright$}};
  \vertex{C}{2};
  \node at (1,0.6) { };
}

\newcommand{\CondensateTypeTwoPiPi}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (C2) at ($(C)+(\len,0)$);
  \coordinate (C3) at ($(C2)+(\len,0)$);
  \coordinate (D) at ($(C)+(0,-0.6)$);
  \draw[source] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[pion] (C) -- (C2);
  \draw[source] (C2) -- (C3);
  \draw[inmedium] ($(C)!0.5!(D)$) circle (.3cm);
  \node at (D) {\scalebox{0.7}{$\blacktriangleright$}};
  \vertex{C}{2};
  \node at (1,0.6) { };
}

\newcommand{\CondensateTypeThree}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A) + (\len,0)$);
  \coordinate (C) at ($(B) + (\len,0)$);
  \coordinate (E) at ($(B) + (-\len*0.7,-\len)$);
  \coordinate (F) at ($(B) + (\len*0.7,-\len)$);
  \draw[source] (A) -- (B);
  \draw[source] (B) -- (C);
  \draw[pion] (B) to[in=90,out=220] (E);
  \draw[pion] (F) to[in=320,out=90] (B);
  \draw[inmedium] (E) to[in=135,out=45] (F);
  \draw[inmedium] (E) to[in=225,out=-45] (F);
  \node at ($(E)!0.5!(F) + (0,0.3)$) {\scalebox{0.7}{$\blacktriangleright$}};
  \node at ($(E)!0.5!(F) + (0,-0.3)$) {\scalebox{0.7}{$\blacktriangleleft$}};
}

\newcommand{\CondensateTypeThreePi}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A) + (\len,0)$);
  \coordinate (C) at ($(B) + (\len,0)$);
  \coordinate (C2) at ($(C) + (\len,0)$);
  \coordinate (E) at ($(B) + (-\len*0.7,-\len)$);
  \coordinate (F) at ($(B) + (\len*0.7,-\len)$);
  \draw[source] (A) -- (B);
  \draw[source] (C) -- (C2);
  \draw[pion] (B) -- (C);
  \draw[pion] (B) to[in=90,out=220] (E);
  \draw[pion] (F) to[in=320,out=90] (B);
  \draw[inmedium] (E) to[in=135,out=45] (F);
  \draw[inmedium] (E) to[in=225,out=-45] (F);
  \node at ($(E)!0.5!(F) + (0,0.3)$) {\scalebox{0.7}{$\blacktriangleright$}};
  \node at ($(E)!0.5!(F) + (0,-0.3)$) {\scalebox{0.7}{$\blacktriangleleft$}};
  \vertex{C}{2};
}

\newcommand{\CondensateTypeThreePiPi}[0]{
  \coordinate (A) at (0,0);
  \coordinate (Z) at ($(A) - (\len,0)$);
  \coordinate (B) at ($(A) + (\len,0)$);
  \coordinate (C) at ($(B) + (\len,0)$);
  \coordinate (C2) at ($(C) + (\len,0)$);
  \coordinate (E) at ($(B) + (-\len*0.7,-\len)$);
  \coordinate (F) at ($(B) + (\len*0.7,-\len)$);
  \draw[source] (Z) -- (A);
  \draw[pion] (A) -- (B);
  \draw[source] (C) -- (C2);
  \draw[pion] (B) -- (C);
  \draw[pion] (B) to[in=90,out=220] (E);
  \draw[pion] (F) to[in=320,out=90] (B);
  \draw[inmedium] (E) to[in=135,out=45] (F);
  \draw[inmedium] (E) to[in=225,out=-45] (F);
  \node at ($(E)!0.5!(F) + (0,0.3)$) {\scalebox{0.7}{$\blacktriangleright$}};
  \node at ($(E)!0.5!(F) + (0,-0.3)$) {\scalebox{0.7}{$\blacktriangleleft$}};
  \vertex{C}{2};
}

\newcommand{\CondensateTypeFour}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (D) at ($(C)+(\len,0)$);
  \draw[source] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[source] (C) -- (D);
  \draw[inmedium] ($(B)!0.5!(C)$) circle (.5cm);
  \node at ($(B)!0.5!(C) + (0,0.5)$) {\scalebox{0.7}{$\blacktriangleright$}};
  \node at ($(B)!0.5!(C) - (0,0.5)$) {\scalebox{0.7}{$\blacktriangleleft$}};
}

\newcommand{\CondensateTypeFourPi}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (D) at ($(C)+(\len,0)$);
  \coordinate (E) at ($(D)+(\len,0)$);
  \draw[source] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[pion] (C) -- (D);
  \draw[source] (D) -- (E);
  \draw[inmedium] ($(B)!0.5!(C)$) circle (.5cm);
  \node at ($(B)!0.5!(C) + (0,0.5)$) {\scalebox{0.7}{$\blacktriangleright$}};
  \node at ($(B)!0.5!(C) - (0,0.5)$) {\scalebox{0.7}{$\blacktriangleleft$}};
  \vertex{D}{2};
}

\newcommand{\CondensateTypeFourPiPi}[0]{
  \coordinate (A) at (0,0);
  \coordinate (Z) at ($(A)-(\len,0)$);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (D) at ($(C)+(\len,0)$);
  \coordinate (E) at ($(D)+(\len,0)$);
  \draw[source] (Z) -- (A);
  \draw[pion] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[pion] (C) -- (D);
  \draw[source] (D) -- (E);
  \draw[inmedium] ($(B)!0.5!(C)$) circle (.5cm);
  \node at ($(B)!0.5!(C) + (0,0.5)$) {\scalebox{0.7}{$\blacktriangleright$}};
  \node at ($(B)!0.5!(C) - (0,0.5)$) {\scalebox{0.7}{$\blacktriangleleft$}};
  \vertex{A}{2};
  \vertex{D}{2};
}

\newcommand{\CondensateTypeFive}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (D) at ($(B)+(0,-\len)$);
  \draw[source] (A) -- (B);
  \draw[source] (B) -- (C);
  \draw[pion] (D) -- (B);
  \draw[inmedium] ($(B)!0.5!(D)$) circle (\len/2);
  \node at ($(B)!0.5!(D) + (\len/2,0)$) {\scalebox{0.7}{$\blacktriangledown$}};
  \node at ($(B)!0.5!(D) - (\len/2,0)$) {\scalebox{0.7}{$\blacktriangle$}};
}

\newcommand{\CondensateTypeFivePi}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (C2) at ($(C)+(\len,0)$);
  \coordinate (D) at ($(B)+(0,-\len)$);
  \draw[source] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[source] (C) -- (C2);
  \draw[pion] (D) -- (B);
  \draw[inmedium] ($(B)!0.5!(D)$) circle (\len/2);
  \node at ($(B)!0.5!(D) + (\len/2,0)$) {\scalebox{0.7}{$\blacktriangledown$}};
  \node at ($(B)!0.5!(D) - (\len/2,0)$) {\scalebox{0.7}{$\blacktriangle$}};
  \vertex{C}{2};
}

\newcommand{\CondensateTypeFivePiPi}[0]{
  \coordinate (A) at (0,0);
  \coordinate (Z) at ($(A)-(\len,0)$);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (C2) at ($(C)+(\len,0)$);
  \coordinate (D) at ($(B)+(0,-\len)$);
  \draw[source] (Z) -- (A);
  \draw[pion] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[source] (C) -- (C2);
  \draw[pion] (D) -- (B);
  \draw[inmedium] ($(B)!0.5!(D)$) circle (\len/2);
  \node at ($(B)!0.5!(D) + (\len/2,0)$) {\scalebox{0.7}{$\blacktriangledown$}};
  \node at ($(B)!0.5!(D) - (\len/2,0)$) {\scalebox{0.7}{$\blacktriangle$}};
  \vertex{A}{2};
  \vertex{C}{2};
  %\node at (0,\len) { };
}









\newcommand{\SUThreeDiagOne}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (C2) at ($(C)+(\len,0)$);
  \coordinate (D) at ($(B)+(0,-0.6)$);
  \draw[source] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[source] (C) -- (C2);
  \draw[inmedium] ($(B)!0.5!(D)$) circle (.3cm);
  \node at (D) {\scalebox{0.7}{$\blacktriangleright$}};
  \vertex{C}{ };
  \node at (1,0.6) { };
}

\newcommand{\SUThreeDiagTwo}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (C2) at ($(C)+(\len,0)$);
  \coordinate (D) at ($(C)+(0,-0.6)$);
  \draw[source] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[source] (C) -- (C2);
  \draw[inmedium] ($(C)!0.5!(D)$) circle (.3cm);
  \node at (D) {\scalebox{0.7}{$\blacktriangleright$}};
  \vertex{C}{ };
  \node at (1,0.6) { };
}

\newcommand{\SUThreeDiagThree}[0]{
  \coordinate (A) at (0,0);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (C2) at ($(C)+(\len,0)$);
  \coordinate (C3) at ($(C2)+(\len,0)$);
  \coordinate (D) at ($(C)+(0,-0.6)$);
  \draw[source] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[pion] (C) -- (C2);
  \draw[source] (C2) -- (C3);
  \draw[inmedium] ($(C)!0.5!(D)$) circle (.3cm);
  \node at (D) {\scalebox{0.7}{$\blacktriangleright$}};
  \vertex{C}{ };
  \node at (1,0.6) { };
}

\newcommand{\SUThreeDiagFour}[0]{
  \coordinate (A) at (0,0);
  \coordinate (Z) at ($(A)-(\len,0)$);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (C2) at ($(C)+(\len,0)$);
  \coordinate (D) at ($(C)+(0,-0.6)$);
  \draw[source] (Z) -- (A);
  \draw[pion] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[source] (C) -- (C2);
  \draw[inmedium] ($(C)!0.5!(D)$) circle (.3cm);
  \node at (D) {\scalebox{0.7}{$\blacktriangleright$}};
  \vertex{C}{ };
  \node at (1,0.6) { };
}

\newcommand{\SUThreeDiagFive}[0]{
  \coordinate (A) at (0,0);
  \coordinate (Z) at ($(A)-(\len,0)$);
  \coordinate (B) at ($(A)+(\len,0)$);
  \coordinate (C) at ($(B)+(\len,0)$);
  \coordinate (C2) at ($(C)+(\len,0)$);
  \coordinate (D) at ($(A)+(0,-0.6)$);
  \draw[source] (Z) -- (A);
  \draw[pion] (A) -- (B);
  \draw[pion] (B) -- (C);
  \draw[source] (C) -- (C2);
  \draw[inmedium] ($(A)!0.5!(D)$) circle (.3cm);
  \node at (D) {\scalebox{0.7}{$\blacktriangleright$}};
  \vertex{C}{ };
  \node at (1,0.6) { };
}
